Ups and downs: Copepods reverse the near-body flow to cruise in the water column

Copepods participate in large-scale diel vertical migrations (DVM) as primary consumers in marine ecosystems. Given that they are negatively buoyant, gravity facilitates their downward cruising but impedes their upward relocation. In principle, overcoming this retarding force using drag-based propulsion during upward swimming incurs extra energy costs that neutrally buoyant or gravity-assisted downward swimmers fundamentally avoid. This added power requirement seemingly renders upward swimming disproportionally less efficient than downward swimming. However, we found a compensatory mechanism enhancing thrust in upward-swimming copepods. Using experimentally derived velocity and pressure fields, we observed that copepods pull water to the anterior, generating sub-ambient pressure gradients when cruising upwards, thereby inducing an upstream suction force to complement the thrust produced by the legs. Contrary to expectations that drag forces always dominate the leg recovery phase, the results show that the upstream suction generates net thrust for about a third of the recovery stroke. Such a suction-thrust mechanism promotes cost-effective swimming in larger animals like fish and jellyfish. However, it has never been reported at small scales. We compare these results with downward-swimming copepods that push rather than pull on water and demonstrate they do not benefit from thrust-enhancing suction effects during the recovery stroke. Instead, downward cruisers leverage gravitational effects to swim faster. `Puller' and `pusher' behaviors are driven by alterations of the leg kinematics, indicating a response to the body orientation rather than a fixed organism trait. These results offer insights into an essential swimming mechanism that can inform us about the role of mesozooplankton in driving biogenic hydrodynamic transport and its effects on marine biogeochemistry.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
